Deep Multitask Learning for Semantic Dependency Parsing

We present a deep neural architecture that parses sentences into three semantic dependency graph formalisms. By using efficient, nearly arc-factored inference and a bidirectional-LSTM composed with a multi-layer perceptron, our base system is able to significantly improve the state of the art for semantic dependency parsing, without using hand-engineered features or syntax. We then explore two multitask learning approaches---one that shares parameters across formalisms, and one that uses higher-order structures to predict the graphs jointly. We find that both approaches improve performance across formalisms on average, achieving a new state of the art. Our code is open-source and available at https://github.com/Noahs-ARK/NeurboParser.

==> text/experiment.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{Experimental Settings}
\label{subsec:experiment:setup}
\noindent\textbf{Compared Methods.}\ \ 
We directly compare our models to two state-of-the-art systems, \citet{du2015sdp} and \citet{almeida2015sdp}.
\citet{du2015sdp} relies on graph-tree transformation techniques proposed in \citet{du2014sdp}, and applies voting-based ensemble to well-studied syntactic parsers.
Closely related to our single-task model is \citet{almeida2015sdp}, where they
use rich second-order features and \adcubed\ for inference.
We also briefly dicuss \citet{kanerva2015sdp}, the only gold-track system we are aware of.\\

\noindent\textbf{Model variants.}\ \ 
Besides the single-task model (basic model), we also compare four multi-task
variants:
\begin{itemize}[leftmargin=*]
\item\texttt{ph1} is a first-order model. It uses $\bm{\phi}$ defined in
Equation \ref{eq:phi_multitask} as its input representation function, i.e., it
only uses a single BiLSTM encoder shared across tasks.
\item\texttt{ph2} is a first-order model. Different from \texttt{ph1}, its input
representation function is $\widetilde{\bm{\phi}}$ (Equation
\ref{eq:phi_multitask_}), i.e., it uses additional task-specific encoders.
\item\texttt{ph3} is a third-order model equipped with cross-task factors. It
follows \texttt{ph1} and uses $\bm{\phi}$ as its representation function, but
employs cross-task inference.
\item \texttt{ph4} is a third-order model. It combines \texttt{ph2} and \texttt{ph3} by using $\widetilde{\bm{\phi}}$ and cross-task factors.
\end{itemize}

\begin{table}[tb]
\small
\center
		\begin{tabulary}{0.47\textwidth}{c |  c c c | c} 
			
			& \textbf{DM}
			& \textbf{PAS}
			& \textbf{PSD}
			& \textbf{Avg.}\\
			
			\hline
			Basic Model
			& 89.4 &  92.2
			& 77.6 & 87.4 \\
			
			\texttt{ph1}
			& 89.7 &  91.9
			& 77.8 & 87.4 \\
			
			\texttt{ph2}
			& 90.0 &  92.3
			& 78.1 & 87.7\\
			
			\texttt{ph3}
			& \ul{\textbf{90.3}} &  \textbf{92.5}
			& \ul{\textbf{78.5}} & \ul{\textbf{88.0}}\\
			
			\texttt{ph3}
			&  &  
			&  & \\
			
			\hline\hline
			
			Du et al. 2015
			& 89.1 &  91.3
			& 75.7 & 86.3 \\
			
			A \& M 2015 (closed)
			& 88.2 &  90.9
			& 76.4 & 86.0 \\
			
			A \& M 2015 (open)$^\dagger$
			& 89.4 &  91.7
			& 77.6 & 87.1 \\
			
			Kanerva et al. 2015$^{\dagger\dagger}$
			& 88.3 &  \ul{95.6}
			& 76.6 & \ul{88.0} \\
			
			
		\end{tabulary}
	\caption{Labeled semantic dependency parsing performance
          ($\mathrm{F}_1$ score) on in-domain test data of SemEval 2015 Task 18. The last column shows the micro-average over the three tasks. $\dagger$ denotes the use of machine generated syntactic analysis, while $\dagger\dagger$ denotes using gold syntactic analysis. Bold font indicates best performance without gold syntactic parse, and best numbers among all are underlined.} 
	\label{tab:res_id_lf}
\end{table}

\begin{table}[tb]
\small
\center
		\begin{tabulary}{0.47\textwidth}{c | ccc|c } 
			
			& \textbf{DM}
			& \textbf{PAS}
			& \textbf{PSD}
			& \textbf{Avg.}\\
			
			\hline
			Basic Model
			& 84.5 &  88.3
			& 75.3 & 83.6 \\
			
			\texttt{ph1}
			& 84.4 &  88.1
			& 75.4 & 83.5 \\
			
			\texttt{ph2}
			& 84.9 &  88.3
			& 75.8 & 83.9\\
			
			\texttt{ph3}
			& \ul{\textbf{85.3}} &  \textbf{88.4}
			& 76.1 & \textbf{84.1}\\
			
			\texttt{ph3}
			&  &  
			&  & \\
			
			\hline\hline
			
			Du et al. 2015
			& 81.8 &  87.2
			& 73.3 & 81.7 \\
			
			A \& M 2015 (closed)
			& 81.8 &  86.9
			& 74.8 & 82.0 \\
			
			A \& M 2015 (open)$^\dagger$
			& 83.8 &  87.6
			& \ul{\textbf{76.2}} & 83.3 \\
			
			Kanerva et al. 2015$^{\dagger\dagger}$
			& 82.1 &  \ul{92.9}
			& 75.5 & \ul{84.8} \\
			
		\end{tabulary}
	\caption{Labeled semantic dependency parsing performance
          ($\mathrm{F}_1$ score) on out-of-domain test data of SemEval
          2015 Task 18. The last column shows the micro-average over the three tasks. $\dagger$ denotes the use of machine generated syntactic analysis, while $\dagger\dagger$ denotes using gold syntactic analysis. Bold font indicates best performance without gold syntactic parse, and best numbers among all are underlined.} 
	\label{tab:res_ood_lf}
\end{table}

\subsection{Empirical Results}
\noindent\textbf{Main results overview.}\ \ 
Tables \ref{tab:res_id_lf} compares our models to best published
results (labeled $\mathrm{F}_1$ score) on SemEval 2015 Task 18 in-domain test data.
Numbers of previous works are taken from official evaluation results.\footnote{\url{http://alt.qcri.org/semeval2015/task18/}}
The micro-averaged scores shown in the last column are calculated using the precision and recall numbers.

In the sense that no syntactic information is used, most comparable models to ours are \citet{du2015sdp} and closed track \citet{almeida2015sdp}.
As shown in the table, even our single-task basic model significantly
outperforms both systems.
Benefiting from multi-task learning, three of the four multi-task variants further improve over the basic model, and outperform previous state-of-the-art systems with substantial absolute improvements of up to 1.7\%.

How semantic dependency parsing benefits from high-quality syntax information remains unclear.
With automatically generated syntactic parses, \citet{almeida2015sdp} manages to obtain more than $1\%$ absolute improvements, which is consistent with the extensive evaluation by \citet{zhang2016transition}.
With gold-standard syntax parses, \citet{kanerva2015sdp} observe further 2\% to 5\% absolute improvements.\footnote{With machine-generated syntactic parses, \citet{kanerva2015sdp} get 86.2, 90.6, and 73.6 labeled $\mathrm{F}_1$ for DM, PAS, and PSD, respectively.}
In practice, high-quality syntactic analysis may not be available.
Therefore, we design our models to not rely on any syntax information.
Although it's less comparable, our basic model is able to achieve similar or stronger performance than open track \citet{almeida2015sdp}, and the multi-task models yield 0.6\% to 0.9\% absolute improvements.
Notably, all of our models outperform \citet{kanerva2015sdp} on two of the three tasks.

On the out-of-domain test set (results shown in Table  \ref{tab:res_ood_lf}), all systems' performance significantly degrades. 
The overall trends are similar, with a notable exception that our best-performing model is slightly behind open track \citet{almeida2015sdp} on PSD.\\


\noindent\textbf{Effects of structural diversions.}\ \ 
Table \ref{tab:structrual_similarity} compares the structural similarities between three formalisms in unlabeled $\mathrm{F}_1$ score.
All three formalisms have more than 55\% overlap when ignoring the arc directions.
Regarding directed similarities, DM and PAS are much closer to each other than either of them to PSD, i.e., PSD tends to have arcs of reversed directions.
Table \ref{tab:res_id_ulf} shows different multi-task models' performance in both unlabeled and labeled $\mathrm{F}_1$ scores and aims to compare how they are effected by the structural diversions of the three formalisms.
Albeit that \texttt{ph1} yields little improvements in labeled performance, we do observe that parameter sharing helps in recovering semantic dependency graph structures.
Interestingly, \texttt{ph3}'s unlabeled performance on PSD \textit{degrades} from its most comparable multi-task baseline \texttt{ph1}.
We think this is due to the directionality differences between PSD on the one
hand, and DM and PAS on the other.
Arcs in a cross-task factor are of the same direction, and thus the cross-task factors may bring additional difficulties to the unlabeled parsing of PSD.
Yet, \texttt{ph3} brings a 0.7\% absolute improvement in labeled $\mathrm{F}_1$ score on PSD.
It may help to deal with the structural diversion issue by allowing arcs of opposite directions in the cross-task factors.
We leave it to future work, though.

\begin{table}[tb]
\center
		\begin{tabulary}{0.47\textwidth}{C | CCC | CCC } 
			& \multicolumn{3}{c}{\textbf{Undirected}}
			& \multicolumn{3}{c}{\textbf{Directed}}\\
			
			& DM & PAS & PSD
			& DM & PAS & PSD\\			
			\hline
			
			DM
			& - & 67.2 & 56.8
			& - &  64.2 & 26.1\\
			
			PAS
			& 70.0 & - & 54.9
			& 66.9 &  - & 26.1\\
			
			PSD
			& 57.4 & 56.3 & -
			& 26.4 &  29.6 & -\\			
		\end{tabulary}
	\caption{Pairwise structural similarities between three formalisms in unlabeled $\mathrm{F}_1$ score. Numbers taken from \citet{oepen2015sdp}} 
	\label{tab:structrual_similarity}
\end{table}


\begin{table}[tb]
\footnotesize
\center
		\begin{tabulary}{0.47\textwidth}{c | CC CC CC } 
			
			& \multicolumn{2}{c}{\textbf{DM}}
			& \multicolumn{2}{c}{\textbf{PAS}}
			& \multicolumn{2}{c}{\textbf{PSD}}\\
			
			& UF & LF
			& UF & LF
			& UF & LF\\
			
			\hline
			
			\texttt{ph1}
			& 91.1 &  89.7
			& 93.1 & 91.9 
			& 88.8 & 77.8\\
			
			\texttt{ph2}
			& 91.4 &  90.0
			& 93.5 & 92.3
			& 88.6 & 78.1\\
			
			\texttt{ph3}
			& 91.5 &  90.3
			& 93.7 & 92.5
			& 87.8 & 78.5\\
			
			\texttt{ph3}
			&  &  
			&  & \\
			
			\hline\hline
			
			Basic Model
			& 90.7 & 89.4
			& 93.4 & 92.2
			& 86.6 & 77.6 \\
			
		\end{tabulary}
	\caption{Both unlabeled (UF) and labeled (LF) parsing
          performance on in-domain test data of SemEval 2015 Task 18.} 
	\label{tab:res_id_ulf}
\end{table}

\begin{comment}
\begin{table*}[tb]
\scriptsize
	\begin{center}
		\begin{tabulary}{\textwidth}{C | C | C | CC  C  CC  C  CC  C  CC} 
			
			\Xhline{1pt}
			& &
			& \multicolumn{2}{c}{\textbf{DM}}
			& \multicolumn{1}{c}{}
			& \multicolumn{2}{c}{\textbf{PAS}}
			& \multicolumn{1}{c}{}
			& \multicolumn{2}{c}{\textbf{PSD}}
			& \multicolumn{1}{c}{}
			& \multicolumn{2}{c}{\textbf{Overall}} \\
			
			\textbf{Domain}& \textbf{System} & \textbf{Method} 
			& UF & LF 
			& & UF & LF      
			& & UF & LF 
			& & UF & LF    \\ 
			\hline\hline
			
			\multirow{8}{*}{id}
			& Lisbon & 2nd-order, \adcubed, closed track
			& 89.5 & 88.2  
			& & 92.1 & 90.9
			& & 87.2 & 76.4
			& & 90.0 & 86.0 \\
			
			& Lisbon & 2nd-order, \adcubed, open track
			& 90.5 & 89.4 
			& & 92.7 & 91.7
			& & 88.6 & 77.6
			& & 90.9 & 87.1 \\
			
			& Peking & tree-graph transformation, parser ensemble
			& 90.5 & 89.1
			& & 92.4 & 91.3
			& & 88.7 & 75.7
			& & 90.8 & 86.3 \\
			
			& This work & single-task,  1st-order
			& 90.7 &  89.4
			& & 93.4 & 92.2
			& &  86.6 & 77.6
			& &  90.7 & 87.4 \\
			
			& This work & multi-task, 1st-order, shared BiLSTM
			& 91.1 &  89.7
			& & 93.1 & 91.9
			& &  88.8 & 77.8
			& &  91.3 & 87.4 \\
			
			& This work & multi-task, 1st-order, frustratingly easy
			& 91.4 &  90.0
			& & 93.5 & 92.3
			& &  88.6 & 78.1
			& &  91.5 & 87.7 \\
			
			& This work & multi-task, 3rd-order, shared BiLSTM
			& 91.5 & \textbf{90.3}
			& & \textbf{93.7} & \textbf{92.5}
			& & 87.8 & \textbf{78.5}
			& & 91.4 & \textbf{88.0} \\
			
			& This work & multi-task, 3rd-order, frustratingly easy
			& \textbf{91.6} & 90.2
			& & 93.4 & 92.2
			& & \textbf{89.1} & 77.9
			& & \textbf{91.6} &  87.6 \\
			\hline\hline
			
			
			
			\multirow{8}{*}{ood}
			& Lisbon & 2nd-order model, \adcubed, closed track
			& 83.6 & 81.8 
			& & 88.5 & 86.9
			& & 84.0 & 74.8
			& & 85.8 & 82.0 \\
			
			& Lisbon & 2nd-order model, \adcubed, open track
			& 85.5 & 83.8 
			& & 89.2 & 87.6
			& & 85.5 & 76.2
			& & 87.0 & 83.3 \\
			
			& Peking & tree-graph transformation, parser ensemble
			& 84.1 & 81.8  
			& & 88.9 & 87.2
			& & 85.7 & 73.3
			& & 86.5 & 81.7 \\
			
			& This work & single-task,  1st-order
			& 86.3 & 84.5  
			& & 89.9 & 88.3
			& & 83.3 & 75.3
			& & 87.0 & 83.6\\
			
			& This work & multi-task, 1st-order, shared BiLSTM
			& 86.4 & 84.4  
			& & 89.7 & 88.1 
			& & 85.5 & 75.4
			& & 87.5 & 83.5 \\
			
			& This work & multi-task, 1st-order, frustratingly easy
			& 86.8 & 84.9  
			& & 90.0 & 88.3
			& & 85.6 & 75.8
			& & 87.8 & 83.9 \\
			
			& This work &  multi-task, 3rd-order, shared BiLSTM
			& \textbf{86.8} & \textbf{85.0}  
			& & \textbf{90.0} & \textbf{88.4}
			& & 84.2 & \textbf{76.0}
			& & 87.5 & \textbf{84.0} \\
			
			& This work & multi-task, 3rd-order, frustratingly easy
			& 86.7 & 85.0
			& & 90.0 & 88.4 
			& & 86.2 & 75.7
			& & 87.9 & 83.8 \\
			\Xhline{1pt}
			
		\end{tabulary}
	\end{center}
	\caption{The results might be updated. Experimental results on
          test set. Only state-of-the-art systems are listed. The
          numbers of Lisbon \citep{almeida2015sdp} and Peking
          \citep{du2015sdp} are taken from official evaluation results
          by SemEval 2015. \nascomment{suggestion for boldface
            convention:  boldface any of our numbers that are higher
            than previous state of the art.  apply significance tests sparingly
            and use an asterisk to mark those results (which need to
            be explained in this caption}} 
	\label{tab:result} 
	\vspace{-.25cm}
\end{table*}
\end{comment}

==> text/formulation.tex <==
\section{Problem Formulation}
\label{sec:formulation}
We treat each semantic formalism as a separate task, and pose parsing to
multiple formalisms as a multitask learning problem.
We start with basic notation, and then formalize single-SDP as a graph parsing
problem.
Its multitask counterpart is then introduced as a problem of predicting
a general directed \textit{multigraph}.

\subsection{Basic Notation} 
We use lowercase boldface letters (e.g., $\bm{v}$, $\bm{x}$) to denote vectors, and denote the concatenation of them as $\left[\bm{v}; \bm{x}\right]$.
Matrices are written using uppercase boldface letters (e.g., $\bm{U}$). We use the superscript $t$ to indicate the $t$th task (e.g., $y^{(t)}$), and there are $m$ tasks in total. 
We use a function $\tau(s)$ to map a \textit{first-order} factor to index set $\left\{t\right\}_{t=1}^{m}$, i.e., $\tau$ returns the index of the task $s$ belongs to. 
\stcomment{We haven't talked about what a first-order factor is yet.} 
Function $\globalscore_{\theta^{(t)}}$ is a instantiation of $\globalscore$ with parameters $\theta^{(t)}$, and is written into $\globalscore^{(t)}$ for shorthand.

We denote the span of consecutive words from $i$ to $j$ (inclusive) as $w_{i:j}$, and we assume access to its POS tag sequence $p_{i:j}$.\footnote{In this work gold-standard tag sequences are provided in the dataset.} 
\stcomment{bold, cuz it's multiple words/tags} 
\hpcomment{I used bolded lower case to denote vectors
  already. $w_{i:j}$ is supposed to be a sequence of scalars, and
  $\bm{w}_{i:j}$ is a sequence of vectors.}
\nascomment{I like bold for any sequence whether of words or reals}
%Given a sentence with $n$ words $w_{1:n}$, we refer to predicate $w_i$ as $\predicate{i}$. 
%An arc with predicate $w_i$, and argument $w_j$ is denoted as $\edge{i}{j}$.
%Similarly, we denote a labeled arc with label $\ell$ as $\ledge{i}{j}{\ell}$. 

\subsection{Semantic Dependency Parsing (SDP)}
This section discusses single-task SDP, and we assume the task index $t$ is
given.
Different from the tree structures in syntactic parsing, a semantic dependency
parse is a directed acyclic graph (DAG).
Each arc in task $t$ has a label from a predefined set $\mathcal{L}^{(t)}$,
indicating the semantic relation of the child to the head. 
Given input sentence $w = w_{1:n}$, semantic dependency parsing aims to find a semantic graph that maximizes a score
function:
\begin{equation}
\hat{y}^{(t)} = \argmax{y \in\mathcal{Y}^{(t)}(w)} F^{(t)}(w, y), 
\label{eq:score}
\end{equation}
where $\mathcal{Y}^{(t)}(w)$ is the set of valid semantic graphs for task $t$ over $w$. 
We assume that $F^{(t)}$ decomposes into a sum of local scores for substructures
in the graph:
\begin{equation}
F^{(t)}(w, y^{(t)}) = \sum_{s \in y^{(t)}} {
f(s), 
}
\label{eq:score_decomposed}
\end{equation}
where $f^{(t)}$ is the local score function for task $t$. 
For notation simplicity, we omit the dependence of $f$ on
$w$ and do not distinguish a graph and its substructure set. 
We write $f$ in a task-agnostic way, but the scoring strategies for different tasks may differ in practice.
\stcomment{not sure what this means.} 
\hpcomment{$f$ is supposed to distinguish the tasks of input
  structures. so we don't need to define a $f^{(t)}$ for each task.}

\nascomment{this is the place to define the first-order version, and
  any ``nearly'' first-order versions we plan to explore.  I would get
all of this out of the way first, before turning to multitask, then
explain what additional higher-order factors we might consider in
multitask parsing.}

\subsection{Multitask Parsing}
\label{subsec:formulation:multi}
%Our first-order model factors over two types of substructures, predicates and arcs:
%\begin{equation}
%\small
%F_{1}^{(t)}(w, y^{(t)}) = \sum_{p \in y^{(t)}} {f^{(t)}(p)} + \sum_{\ledge{i}{j}{\ell} \in y^{(t)}} {
%f^{(t)}(\ledge{i}{j}{\ell}), 
%}
%\label{eq:1st_order}
%\end{equation}
%where $p$ denotes predicate substructure.
So far we've discussed single-task SDP, but the model can be easily
generalized to the multitask learning scenario.
Suppose the model deals with $m$ different tasks simultaneously (in our
experiments $m=3$), then its task is to predict $m$ graphs
$\{y^{(t)}\}_{t=1}^{m}$ for a given input sentence $w$. Multitask parsing can also be understood as parsing $w$ into a single unified  \textit{multigraph}
$y = \bigcup_{i=1}^{m}y^{(t)}$. %, where there can be up to $m$ arcs between a
% pair of vertices, since it is essentially an union of $m$ DAGs.
To obtain the score for a multigraph $y$, we simply sum the scores
of each task: % (from Equation \ref{eq:arc_factored}):
\begin{equation}
F(w, y) = \sum_{t=1}^{m}F^{(t)}\bigl(w, y^{(t)}\bigr).
\label{eq:multi_score}
\end{equation}
%Note that if each $F^{(t)}$ is of first-order as $F_{1}^{(t)}$ in
%Equation \ref{eq:1st_order}, then so is $F$.
Multitask SDP can then be formalized as finding the union of graphs that
maximizes:
\begin{equation}
\hat{y} = \argmax{y \in\mathcal{Y}(w)}F(w, y), 
\label{eq:multi_task}
\end{equation}
where $\mathcal{Y}(w) = \bigl\{\bigcup_{t=1}^{m}y^{(t)} \mid y^{(t)} \in \mathcal{Y}^{(t)}(w), t = 1, 2, \ldots, m\bigr\}$.
%\mathcal{Y}^{(1)}(w) \times \mathcal{Y}^{(2)}(w) \times \cdots \mathcal{Y}^{(m)}(w) \times \}$. \\ %\in \{1, 2, \dots, m\}\}$.  \\
\begin{comment}
\subsection{Higher-order Factors} 
In syntactic parsing, higher order factors have commonly been used to
model interactions between multiple adjacent arcs in the same dependency tree
\interalia{carreras2007experiments,smith2008dependency,martins2009concise}.
\stcomment{cite Barzilay stuff}.
We use higher-order factors to model small motifs of arcs \textit{across}
different tasks,
analogously to \newcite{lluis2013joint}, who used second-order factors to
jointly model syntactic dependencies and semantic roles.
For us, a $k^{\text{th}}$-order factor is able to score arcs from $k$ of the $m$
formalisms.

\stcomment{move to intro?}
Different annotation styles may capture different syntactic/semantic aspects of the language. Our intuition behind cross-task factors is to utilize the potential similarity between different tasks. \hpcomment{cite the linguistic paper?}

\stcomment{
Cite \cite{lluis2013joint} for second-order factors across tasks.}

\hpcomment{
also introduce the score function for 2nd and 3rd order factors? the readers may expect $s_2$ and $s_3$ when seeing $s_1$}
\end{comment}
